Virtual KITTI 2

This paper introduces an updated version of the well-known Virtual KITTI dataset which consists of 5 sequence clones from the KITTI tracking benchmark. In addition, the dataset provides different variants of these sequences such as modified weather conditions (e.g. fog, rain) or modified camera configurations (e.g. rotated by 15 degrees). For each sequence, we provide multiple sets of images containing RGB, depth, class segmentation, instance segmentation, flow, and scene flow data. Camera parameters and poses as well as vehicle locations are available as well. In order to showcase some of the dataset's capabilities, we ran multiple relevant experiments using state-of-the-art algorithms from the field of autonomous driving. The dataset is available for download at https://europe.naverlabs.com/Research/Computer-Vision/Proxy-Virtual-Worlds.

==> trash.tex <==
\begin{table}[h]
\caption{test\_disp on kitti using different models trained on snippets of 3}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
model   & abs\_diff & abs\_rel & sq\_rel & rms     & log\_rms & abs\_log & a1     & a2     & a3     \\ \hline
kitti Eigen split [ref]  & 3.5348    & 0.2068   & 1.8060  & 6.3873  & 0.2757   & 0.1973   & 0.6983 & 0.8949 & 0.9609 \\ \hline
vkitti  & 6.0451    & 0.3756   & 4.7071  & 9.8582  & 0.4774   & 0.3628   & 0.4219 & 0.7088 & 0.8553 \\ \hline
vkitti2 & 7.2319    & 0.4345   & 4.5384  & 11.8028 & 0.5744   & 0.4523   & 0.3174 & 0.5763 & 0.7751 \\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\caption{test\_disp on vkitti using different models trained on snippets of 3}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
model                       & abs\_diff & abs\_rel & sq\_rel & rms     & log\_rms & abs\_log & a1     & a2     & a3     \\ \hline
kitti Eigen split {[}ref{]} & 4.0614    & 0.1956   & 1.7370  & 7.7066  & 0.2837   & 0.1971   & 0.7010 & 0.8839 & 0.9572 \\ \hline
vkitti                      & 5.4377    & 0.2887   & 8.9938  & 9.7394  & 0.4022   & 0.2825   & 0.6733 & 0.8175 & 0.8819 \\ \hline
vkitti2                     & 9.1056    & 0.4740   & 6.0778  & 14.9506 & 0.6563   & 0.5183   & 0.2699 & 0.5296 & 0.7256 \\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\caption{test\_pose on kitti sequence 09 using different models trained on snippets of 3}
\centering
\begin{tabular}{|l|l|l|}
\hline
model   & ATE              & RE               \\ \hline
kitti Eigen split [ref]   & 0.0151 +- 0.0101 & 0.0030 +- 0.0020 \\ \hline
vkitti  & 0.2627 +- 0.1238 & 0.0117 +- 0.0112 \\ \hline
vkitti2 & 0.3924 +- 0.1524 & 0.0120 +- 0.0114 \\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\caption{test\_pose on vkitti sequence 01 using different models trained on snippets of 3}
\centering

\end{table}
